Standard Gaussian Process is All You Need for High-Dimensional Bayesian Optimization

A long-standing belief holds that Bayesian Optimization (BO) with standard Gaussian processes (GP) -- referred to as standard BO -- underperforms in high-dimensional optimization problems. While this belief seems plausible, it lacks both robust empirical evidence and theoretical justification. To address this gap, we present a systematic investigation. First, through a comprehensive evaluation across twelve benchmarks, we found that while the popular Square Exponential (SE) kernel often leads to poor performance, using Mat\'ern kernels enables standard BO to consistently achieve top-tier results, frequently surpassing methods specifically designed for high-dimensional optimization. Second, our theoretical analysis reveals that the SE kernel's failure primarily stems from improper initialization of the length-scale parameters, which are commonly used in practice but can cause gradient vanishing in training. We provide a probabilistic bound to characterize this issue, showing that Mat\'ern kernels are less susceptible and can robustly handle much higher dimensions. Third, we propose a simple robust initialization strategy that dramatically improves the performance of the SE kernel, bringing it close to state-of-the-art methods, without requiring additional priors or regularization. We prove another probabilistic bound that demonstrates how the gradient vanishing issue can be effectively mitigated with our method. Our findings advocate for a re-evaluation of standard BO's potential in high-dimensional settings.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> theory-Gaussian.tex <==
\section{Theoretical Analysis}\label{sect:theory}
To understand why, in high-dimensional tasks, standard BO with the SE kernel often performs poorly, while achieving excellent results with the Mat\'ern kernel,  we look into the gradient structure during the GP training. Specifically, we consider at the beginning, all the length-scale parameters are set to the same initial value, $\ell_1 = \ldots =\ell_d = \ell_0$. %In practice, $\ell_0$ is often chosen a small constant value, such as $\ell_0 = 1$ or $\ell_0 = 0.5$.  
From the marginal likelihood (~\eqref{eq:gp-ll}), we can obtain the gradient w.r.t each length-scale, 
\begin{align}
    \frac{\partial \log p(\y|\X)}{\partial \ell_k} = \frac{1}{2} \tr\left(\A\cdot\frac{\partial \K}{\partial \ell_k}\right), \label{eq:total-grad}
\end{align}
where $\A = \balpha \balpha^\top - (\K + \sigma^2\I)^{-1}$, $\balpha = (\K + \sigma^2\I)^{-1}\y$, and  each entry of $\frac{\partial \K}{\partial \ell_k}$ is as follows: $\left[\frac{\partial \K}{\partial \ell_k}\right]_{ii}=0$ and for $i \neq j$,
\begin{align}
    &\left[\frac{\partial \K}{\partial \ell_k}\right]_{ij} = \frac{\partial \kappa_{\text{SE}}(\x_i, \x_j)}{\partial \ell_k} = -\frac{2a}{\ell_k} \exp(-\frac{\|\x_i-\x_j\|^2}{\ell_0^2}) \frac{(x_{ik} - x_{jk})^2}{\ell_k^2} \le -\frac{2a}{\ell_k} \cdot \frac{\rho^2}{e^{\rho^2}},\label{eq:grad-se}
\end{align}
where $x_{ik}$ and $x_{jk}$ are the $k$-th element in $\x_i$ and $\x_j$, respectively, and 
$\rho = \frac{\|\x_i - \x_j\|}{\ell_0}$.

Intuitively, as the input dimension $d$ increases, the squared distance between input vectors grows rapidly. Consequently, the factor $\frac{\rho^2}{e^{\rho^2}}$ in \eqref{eq:grad-se} can quickly fall below the machine epsilon $\xi$, causing the gradient in \eqref{eq:grad-se} to vanish.
\begin{lemma}\label{lem:tau-se}
    When $\rho>\tau_{\text{SE}}=\frac{1}{2} + \sqrt{\frac{1}{4} - \log \xi}$, $\frac{\rho^2}{e^{\rho^2}} < \xi$ and $\frac{\partial \kappa_{\text{SE}}(\x_i, \x_j)}{\partial \ell_k}$ becomes zero numerically.  
\end{lemma}
When using the double-precision floating-point format (float64), the rounding machine epsilon is $\xi = 2^{-53}$, and  the above threshold is $\tau_{\text{SE}} = 6.58$. 
To analyze the likelihood of gradient vanishing, we provide a probabilistic bound under Gaussian data assumption. 
\begin{lemma}\label{lem:prob-bound}
    Suppose the input domain is $\mathbb{R}^d$ and each input vector is sampled from the standard Gaussian distribution $\N(\0, \I)$,  then for any constant threshold $\tau>0$, when $d>\ell_0^2\tau^2/2$, 
    \begin{align}
    p(\rho\ge \tau) > 1 - \frac{2d}{\left(d - \frac{1}{2}\ell_0^2\tau^2\right)^2}. \label{eq:bound-prob}
    \end{align}
\end{lemma}
The lower bound is $1 - 1/\mathcal{O}(d)$, which increases with $d$ and converges to one. This implies  that given any $\ell_0$ choice constant to $d$ (\eg $\ell_0=1$), with the growth of the input dimension $d$,  the probability $p(\rho > \tau_{\text{SE}})$ will approach one, causing the gradient vanishing for any pair of the inputs $\x_i$ and $\x_j$. As a consequence, the total gradient w.r.t each length scale $\ell_k$ in \eqref{eq:total-grad} becomes trivial, preventing any effective training\footnote{A union bound can be directly derived from \eqref{eq:bound-prob} to lower bound the joint probability that all gradients $\{\partial \kappa_{\text{SE}}(\x_i, \x_j)/\partial \ell_k\}_{i,j}$  across $N$ training instances are numerically zero. However, this bound  is too loose to reflect our practical observations (see XX). Therefore, we focus our discussion on a single pair of inputs. }. The inferior prediction accuracy of the GP model further contributes to poor performance in the BO procedure. Since  $\tau_\text{SE}$ is quite small,  gradient vanishing can occur even when $d$ is not very large. For example, for $\ell_0=0.5$ and $\ell_0=1$,  we have $p(\rho>\tau_\text{SE}) > 0.99$ when $d\ge 207$ and $d\ge 202$, respectively.  
\zhec{zhitong add experiments to show this; real-data and synthetic } To confirm this issue in practical training, we test on .....

\noindent\textbf{Why Mat\'ern kernels perform  better?} We now apply the same framework to analyze the behavior of GP training with the Mat\'ern kernel as defined in \eqref{eq:matern}. 
First, we obtain the gradient, 
\begin{align}
    \frac{\partial \kappa_{\text{Mat\'ern}}(\x_i, \x_j)}{\partial \ell_k} = \frac{5}{3}(1 +\sqrt{5}\rho) \exp{(-\sqrt{5}\rho)} \frac{(x_{ik} - x_{jk})^2}{\ell_k^3} \notag 
    \le \frac{5(1+\sqrt{5})\rho}{3\ell_k^3} \cdot \frac{\rho^2}{e^{\sqrt{5}\rho}}. 
\end{align}
As the distance increases, the factor $\rho^2/e^{\sqrt{5}\rho}$ will also converge to zero, implying that with the growth of $d$, the gradient will eventually become numerically zero. However, since this factor $\rho^2/e^{\sqrt{5}\rho}$ decreases much slower than the corresponding factor in the SE case, \ie $\rho^2/e^{\rho^2}$ in \eqref{eq:grad-se}, the Mat\'ern kernel is able to robustly handle much higher dimensions.  
\begin{lemma}\label{lem:tau-matern}
    When $\rho>\tau_{\text{Mat\'ern}}=\left(1 + \sqrt{1 + \log 1/5- \log \xi}\right)^2/\sqrt{5}$, $\frac{\rho^2}{e^{\sqrt{5}\rho}} < \xi$ and $\frac{\partial \kappa_{\text{Mat\'ern}}(\x_i, \x_j)}{\partial \ell_k}$ becomes zero numerically.  
\end{lemma}
With the machine epsilon $\xi=2^{-53}$, the threshold $\tau_{\text{Mat\'ern}} = 21.98$, more than $300\%$ larger than $\tau_{\text{SE}}=6.58$. Therefore, to achieve the same lower bound in \eqref{eq:bound-prob}, a much higher $d$ is required for Mat\'ern kernel compared to the SE kernel. It implies that using the same initialization for $\ell_0$, the Mat\'ern kernel is able to robustly handle higher dimensions. For concrete examples, we list the dimension $d$ versus the lower bound in Table~\ref{tb:bound-vs-d}. We further conducted real experiments to confirm the advantage of Mat\'ern kernel in GP learning with high dimensions. \zhec{As shown in ... we can see ... }
 \begin{table}[t]
 \centering
 \small
 \begin{tabular}{c|cccccc} 
 \hline\hline
 Lower bound & 0.95 & 0.99 & 0.995 & 0.999 & 0.9995 & 0.9999\\
 \hline
 SE ($d$) &        78 & 242 & 443 & 2044 & 4043 & 20044 \\
 Mat\'ern ($d$) & 362 & 584 & 812 & 2460 & 4471 & 20481\\
  \hline
 \end{tabular}
 \caption{\small The input dimension $d$ \textit{vs.} lower bound probability of gradient vanishing under $\ell_0=1$.} \label{tb:bound-vs-d}
% %\vspace{-0.3in}
 \end{table}



\section{Robust Initialization}
From the analysis in Section~\ref{sect:theory}, one straightforward approach to improving learning with the SE (and Mat\'ern) kernel is to initialize each length-scale with a larger $\ell_0$, which can loosen the lower bound in \eqref{eq:bound-prob} and allow the GP model to better adapt to higher dimensions. This effectiveness is confirmed in XXX. However, this approach is not robust enough, as $d - \frac{1}{2}\ell_0^2\tau^2$ will continue to increase with $d$, and the bound will still rise toward one, eventually causing the gradient to vanish. To address this issue, we propose setting $\ell_0$ to grow with $d$ rather than keeping it constant, 
\begin{align}
    \ell_0 = c \sqrt{d}, \;\;\; c>0.
\end{align}

\begin{lemma}\label{lem:new-bound}
     Suppose the input domain is $\mathbb{R}^d$ and each input vector is sampled from the standard Gaussian distribution $\N(\0, \I)$.  Given any constant threshold $\tau>0$, we set $\ell_0 = c \sqrt{d}$ such that $c > \frac{\sqrt{2}}{\tau}$, then
     \begin{align}
         p(\rho \ge \tau) \le \frac{8}{(c^2\tau- 2)d}.
     \end{align}
\end{lemma}
With this initialization, the increase in $d$ actually reduces the upper bound on the probability of $\rho$ exceeding the given threshold $\tau$. As a result, the gradient vanishing issue can be fundamentally mitigated in the high-dimensional settings. 

We then tested standard BO using SE kernel with our proposed length-scale initialization where we set $c=1$. As shown in Fig. XXXX, the performance across all the benchmarks is dramatically improved, as compared to using popular initialization $\ell_0 = 1$. The performance matches that of using Mat\'ern kernels, achieving state-of-the-art (or near-best) results. This demonstrates that our method can effectively adapt SE kernels to high-dimensional settings, and eliminate the failure mode of standard BO.

Recent work~\citep{hvarfner2024vanilla} proposes an intuitive heuristics to mitigate the learning challenge of the SE kernel in the high-dimensional spaces by constructing a log-normal prior over each length scale, $p(\ell_k) = \text{LogNormal}(\ell_k|\mu_0 + \frac{\log(d)}{2}, \sigma_0)$. This regularizes the length-scale to be  on the order of $\sqrt{d}$ during training.  Using our theoretical framework, this method can be justified as an alternative strategy to alleviate the gradient vanishing issue. However, it is worth noting that our method,  directly motivated by our analysis, is even simpler --- requiring no additional priors or associated  parameters, and has been shown to be be highly effective. The comparison between~\citep{hvarfner2024vanilla} and our method is given in Appendix Section XXX. 



\section{Proofs}\label{sect:proof}
\subsection{Proof of Lemma~\ref{lem:tau-se} }
\begin{proof}
    We intend to solve $\rho^2/e^{\rho^2} < \xi$, which is equivalent to solving
    \[
     \log r - r < \log \xi, 
    \]
    where $r = \rho^2$. 
    We then leverage the fact that $\log r < \sqrt{r}$ when $r > 1$. Since $1/e > \xi$, we know the solution of $\rho$ must be larger than 1, implying that the solution for $r$ is larger than $1$. To meet the inequality, we can solve 
    \[
    \log r - r < \sqrt{r} - r < \log \xi. 
    \]
    It then converts to a quadratic form, 
    \begin{align}
        \sqrt{r} - \sqrt{r}^2 < \log \xi.
    \end{align}
    Note that $\rho = \sqrt{r}$.     It is straightforward to solve this inequality and we can obtain that the inequality holds when
    \[
    \rho > \tau_{\text{SE}} = \frac{1}{2} + \sqrt{\frac{1}{4} - \log \xi}. 
    \]
    
\end{proof}
\subsection{Proof of Lemma~\ref{lem:prob-bound}}\label{sect:bound-proof-1}
\begin{proof}
    First, we observe that $\|\x_i - \x_j\|^2 = \sum_k (x_{ik} - x_{jk})^2$. Since all $x_{ik}$ and $x_{jk}$ independently follow $\N(0, 1)$, we have each $x_{ik}-x_{jk} \sim \N(0, 2)$, and hence 
    \[
    \frac{1}{\sqrt{2}} (x_{ik} - x_{jk}) \sim \N(0, 1).
    \]
    Let us define $\gamma = \|\x_i - \x_j\|^2$. Then we have
    \[
    \frac{1}{2}\gamma = \frac{1}{2} \sum_{k=1}^d (x_{ik} - x_{jk})^2 \sim \chi^2(d), 
    \]
    from which we immediately obtain
    \begin{align}
        \EE[\gamma] = 2d, \;\;\; \text{Var}(\gamma) = 8d. 
    \end{align}
    From Chebyshev's inequality, we know for all $a>0$,
    \begin{align}
        p(|\gamma - 2d| \ge a) \le  \frac{8d}{a^2}. \label{eq:cheb}
    \end{align}
    Since $\rho = 
    \frac{\sqrt{\gamma}}{\ell_0}$, we have  $p(\rho > \tau) = p(\gamma > \tau^2\ell_0^2)$. Since $d>\frac{\ell_0^2\tau^2}{2}$, we set $a = 2d - \ell_0^2\tau^2>0$, and apply \eqref{eq:cheb} , we obtain
    \[
    p(|\gamma - 2d| \ge 2d -  \ell_0^2\tau^2|) \le \frac{8d}{(2d - \ell_0^2\tau^2)^2}  = \frac{2d}{\left(d - \frac{1}{2}\ell_0^2\tau^2\right)^2},
    \]
    which is equivalent to
    \begin{align}
        p(|\gamma-2d| < 2d - \ell_0^2\tau^2) > 1 - \frac{2d}{\left(d - \frac{1}{2}\ell_0^2\tau^2\right)^2}.\label{eq:bound2}
    \end{align}
Since $p(\gamma > \ell_0^2 \tau^2) \ge p( \ell_0^2 \tau^2 < \gamma < 4d - \ell_0^2 \tau^2) = 
p(|\gamma - 2d| < 2d - \ell_0^2\tau^2)$, combining with \eqref{eq:bound2} we obtain the bound
\[
p(\rho>\tau) = p(\gamma > \ell_0^2 \tau^2) > 1 - \frac{2d}{\left(d - \frac{1}{2}\ell_0^2\tau^2\right)^2}.
\]
\end{proof}

\subsection{Proof of Lemma~\ref{lem:tau-matern}}
\begin{proof}
    To solve $\rho^2/e^{\sqrt{5}\rho} < \xi$, it is equivalent to solving
    \[
    \frac{1}{5} \frac{r^2}{e^r} < \xi, \;\;\; r = \sqrt{5}\rho,
    \]
    which is further equivalent to 
    \[
    \log \frac{1}{5} + 2 \log r - r < \log \xi. 
    \]
    We leverage $\log r < \sqrt{r}$ for $r>1$, and solve the upper bound, 
    \[
    \log\frac{1}{5} + 2 \sqrt{r}-r < \log \xi,
    \]
    which gives 
    \begin{align}
        \rho > \tau_{\text{Mat\'ern}} = \frac{1}{\sqrt{5}}\left(1 + \sqrt{1 + \log 1/5 - \log\xi}\right)^2.
    \end{align}
\end{proof}

\subsection{Proof of Lemma~\ref{lem:new-bound}}
\begin{proof}
    First, similar to the proof in Section~\ref{sect:bound-proof-1}, under standard Gaussian data distribution, we have for all $a>0$, 
    \begin{align}
    p(|\gamma - 2d| \ge a) \le \frac{8d}{a^2}, \label{eq:cheb}
    \end{align}
    where $\gamma = \|\x_i - \x_j\|^2$. Since $\rho = \frac{\sqrt{\gamma}}{\ell_0}$, 
    \[
    p(\rho \ge \tau) = p(\gamma \ge \ell_0^2 \tau^2).
    \]
    When we set $\ell_0 = c\sqrt{d}$ such that $c> \sqrt{2}/\tau$, we have $\ell_0^2 \tau^2 > 2d $. Let us choose $a = \ell_0^2\tau^2 - 2d=c^2 \tau^2d - 2d>0$, and apply the Chebshev's inequality~\eqref{eq:cheb}, 
    \begin{align}
        p(|\gamma - 2d | \ge \ell_0^2\tau^2 - 2d) \le \frac{8d}{(c^2\tau^2d - 2d)^2} = \frac{8}{(c^2\tau^2 -2)d}.
    \end{align}
    Since $p(\rho \ge \tau) = p(\gamma \ge \ell_0^2\tau^2) \le p(|\gamma - 2d | \ge \ell_0^2\tau^2 - 2d)$, we obtain
    \[
    p(\rho \ge\tau) \le \frac{8}{(c^2\tau^2 - 2)d}.
    \]
\end{proof}

